Topology of random 2-dimensional cubical complexes

We study a natural model of random 2-dimensional cubical complex which is a subcomplex of an n-dimensional cube, and where every possible square $2$-face is included independently with probability p. Our main result is to exhibit a sharp threshold p=1/2 for homology vanishing as $n \to \infty$. This is a 2-dimensional analogue of the Burtin and Erd\H{o}s-Spencer theorems characterizing the connectivity threshold for random cubical graphs. Our main result can also be seen as a cubical counterpart to the Linial--Meshulam theorem for random 2-dimensional simplicial complexes. However, the models exhibit strikingly different behaviors. We show that if $p > 1 - \sqrt{1/2} \approx 0.2929$, then with high probability the fundamental group is a free group with one generator for every maximal $1$-dimensional face. As a corollary, homology vanishing and simple connectivity have the same threshold, even in the strong "hitting time" sense. This is in contrast with the simplicial case, where the thresholds are far apart. The proof depends on an iterative algorithm for contracting cycles -- we show that with high probability the algorithm rapidly and dramatically simplifies the fundamental group, converging after only a few steps.

==> Step_1.tex <==
\begin{center}
\begin{tikzpicture}[scale=3,tdplot_rotated_coords,
                    cube/.style={very thick,black},
                    grid/.style={very thin,gray},
                    axis/.style={->,blue,ultra thick},
                    rotated axis/.style={->,purple,ultra thick}]

    %draw the top and bottom of the polycube
    \draw[cube,fill=blue!5] (0,0,0) -- (0,1,0) -- (1,1,0) -- (1,0,0) -- cycle;

    %draw the top and bottom of the polycube
    \draw[cube,fill=blue!5] (0,0,0) -- (0,1,0) -- (0,1,1) -- (0,0,1) -- cycle;

    %draw the top and bottom of the polycube
    \draw[cube,fill=blue!5] (0,0,0) -- (1,0,0) -- (1,0,1) -- (0,0,1) -- cycle;
    
    \draw[cube,fill=red!5] (0,1,0) -- (0,1,1) -- (1,1,1) -- (1,1,0) -- cycle;
    %\draw[cube,fill=red!5] (1,1,0) -- (1,1,1) -- (2,1,1) -- (2,1,0) -- cycle;
    %\draw[cube,fill=red!5] (1,0,0) -- (1,0,1) -- (1,1,1) -- (1,1,0) -- cycle;
   % \draw[cube,fill=red!5] (1,1,0) -- (1,1,1) -- (1,2,1) -- (1,2,0) -- cycle;

\foreach \x in {0,1,1}
   \foreach \y in {0,1,1}
      \foreach \z in {0,1}{
           %#####################################################
           \ifthenelse{  \lengthtest{\x pt < 1pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x+1,\y,\z);
           }
           {% False
           }
           %#####################################################
           \ifthenelse{  \lengthtest{\y pt < 1pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x,\y+1,\z);
           }
           {% False
           }
           %#####################################################
           \ifthenelse{  \lengthtest{\z pt < 1pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x,\y,\z+1);
           }
           {% False
           }
           \shade[rotated axis,ball color = black!80] (\x,\y,\z) circle (0.06cm);          
}

\end{tikzpicture}
\end{center}

==> Step_2.tex <==
\begin{center}
\begin{tikzpicture}[scale=3,tdplot_rotated_coords,
                    cube/.style={very thick,black},
                    grid/.style={very thin,gray},
                    axis/.style={->,blue,ultra thick},
                    rotated axis/.style={->,purple,ultra thick}]

    %draw the top and bottom of the cube
    \draw[cube,fill=blue!5] (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;

    %draw the top and bottom of the cube
    \draw[cube,fill=blue!5] (0,0,0) -- (0,2,0) -- (0,2,1) -- (0,0,1) -- cycle;

    %draw the top and bottom of the cube
    \draw[cube,fill=blue!5] (0,0,0) -- (2,0,0) -- (2,0,1) -- (0,0,1) -- cycle;
    
    \draw[cube,fill=red!5] (0,1,0) -- (0,1,1) -- (1,1,1) -- (1,1,0) -- cycle;
    \draw[cube,fill=red!5] (1,1,0) -- (1,1,1) -- (2,1,1) -- (2,1,0) -- cycle;
    \draw[cube,fill=red!5] (1,0,0) -- (1,0,1) -- (1,1,1) -- (1,1,0) -- cycle;
    \draw[cube,fill=red!5] (1,1,0) -- (1,1,1) -- (1,2,1) -- (1,2,0) -- cycle;

\foreach \x in {0,1,2}
   \foreach \y in {0,1,2}
      \foreach \z in {0,1}{
           %#####################################################
           \ifthenelse{  \lengthtest{\x pt < 2pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x+1,\y,\z);
           }
           {% False
           }
           %#####################################################
           \ifthenelse{  \lengthtest{\y pt < 2pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x,\y+1,\z);
           }
           {% False
           }
           %#####################################################
           \ifthenelse{  \lengthtest{\z pt < 1pt}  }
           {
             % True
                \draw [black]   (\x,\y,\z) -- (\x,\y,\z+1);
           }
           {% False
           }
           \shade[rotated axis,ball color = black!80] (\x,\y,\z) circle (0.06cm);          
}

\end{tikzpicture}
\end{center}

==> cube.tex <==
\begin{tikzpicture}[thick,scale=3]
    \coordinate (A1) at (0, 0);
    \coordinate (A2) at (0, 1);
    \coordinate (A3) at (1, 1);
    \coordinate (A4) at (1, 0);
    \coordinate (B1) at (0.3, 0.3);
    \coordinate (B2) at (0.3, 1.3);
    \coordinate (B3) at (1.3, 1.3);
    \coordinate (B4) at (1.3, 0.3);

    \draw[very thick] (A1) -- (A2);
    \draw[very thick] (A2) -- (A3);
    \draw[very thick] (A3) -- (A4);
    \draw[very thick] (A4) -- (A1);

    \draw[dashed] (A1) -- (B1);
    \draw[dashed] (B1) -- (B2);
    \draw[very thick] (A2) -- (B2);
    \draw[very thick] (B2) -- (B3);
    \draw[very thick] (A3) -- (B3);
    \draw[very thick] (A4) -- (B4);
    \draw[very thick] (B4) -- (B3);
    \draw[dashed] (B1) -- (B4);

    %\draw[fill=yellow,opacity=0.6] (A1) -- (B1) -- (B4) -- (A4);
    \draw[fill=black!20,opacity=0.5] (A1) -- (A2) -- (A3) -- (A4);
    \draw[fill=black!20,opacity=0.6] (A1) -- (A2) -- (B2) -- (B1);
    \draw[fill=black!20,opacity=0.6] (B1) -- (B2) -- (B3) -- (B4);
    \draw[fill=black!20,opacity=0.6] (A3) -- (B3) -- (B4) -- (A4);
    %\draw[fill=green,opacity=0.6] (A2) -- (B2) -- (B3) -- (A3);

\end{tikzpicture}
